The Straw Tracking Detector for the Fermilab Muon $g-2$ Experiment

The Muon $g-2$ Experiment at Fermilab uses a gaseous straw tracking detector to make detailed measurements of the stored muon beam profile, which are essential for the experiment to achieve its uncertainty goals. Positrons from muon decays spiral inward and pass through the tracking detector before striking an electromagnetic calorimeter. The tracking detector is therefore located inside the vacuum chamber in a region where the magnetic field is large and non-uniform. As such, the tracking detector must have a low leak rate to maintain a high-quality vacuum, must be non-magnetic so as not to perturb the magnetic field and, to minimize energy loss, must have a low radiation length. The performance of the tracking detector has met or surpassed the design requirements, with adequate electronic noise levels, an average straw hit resolution of $(110 \pm 20) \,\mu$m, a detection efficiency of 97% or higher, and no performance degradation or signs of aging. The tracking detector's measurements result in an otherwise unachievable understanding of the muon's beam motion, particularly at early times in the experiment's measurement period when there are a significantly greater number of muons decaying. This is vital to the statistical power of the experiment, as well as facilitating the precise extraction of several systematic corrections and uncertainties. This paper describes the design, construction, testing, commissioning, and performance of the tracking detector.

==> TexFiles/acknowledgements.tex <==
{\bf Maybe a sentence mentioning Barry here?}

This work was supported in part by the  Science and Technology
Facilities Council (UK), the European Union's Horizon 2020 research and
innovation programme under the Marie Sk\l{}odowska-Curie grant agreement
No. 690835 (MUSE), the US DOE under contract zyx and Fermilab.

{\bf Did anyone get NSF support ??}

We also thank xx,xxx (e.g. BU undergrads and any non authors who helped) and the staff of the Fermilab Test Beam Facility.

